An EPTAS for Budgeted Matching and Budgeted Matroid Intersection

We study the budgeted versions of the well known matching and matroid intersection problems. While both problems admit a polynomial-time approximation scheme (PTAS) [Berger et al. (Math. Programming, 2011), Chekuri, Vondrak and Zenklusen (SODA 2011)], it has been an intriguing open question whether these problems admit a fully PTAS (FPTAS), or even an efficient PTAS (EPTAS). In this paper we answer the second part of this question affirmatively, by presenting an EPTAS for budgeted matching and budgeted matroid intersection. A main component of our scheme is a novel construction of representative sets for desired solutions, whose cardinality depends only on $\varepsilon$, the accuracy parameter. Thus, enumerating over solutions within a representative set leads to an EPTAS. This crucially distinguishes our algorithms from previous approaches, which rely on exhaustive enumeration over the solution set. Our ideas for constructing representative sets may find use in tackling other budgeted optimization problems, and are thus of independent interest.

==> LP.tex <==
\section{Omitted Proofs}
\label{sec:omitted}

\noindent{\bf Proof of Lemma~\ref{lem:Solution}}: 
As this proof is based on the proof of a corresponding Lemma in \cite{doron2022eptas}, we use some of their definitions and notations. With a slight abuse of notation, 
we use $\OPT$ also to denote the profit of an optimal solution for $I$.
Given an optimal solution, we partition a subset of the elements in the solution 
into $\ceil{\eps^{-1}}$ disjoint sets (some sets may be empty). Specifically,
let $N = \ceil{\eps^{-1}}$; for all $i \in [N]$ define 
\begin{equation}
	\label{J_i}
	J_i = \big\{e \in \OPT~\big|~ p(e) \in \big(\eps^{i} \cdot \OPT(I),  \eps^{i-1} \cdot \OPT(I) \big] \big\}.		
\end{equation} 
Let $i^* = \argmin_{i\in [N]} p(J_i)$. By \eqref{J_i} we have at least 
$\eps^{-1}$ disjoint sets; thus, $p(J_{i^*}) \leq \eps \cdot \OPT(I)$. 
Now, let $L~= ~\bigcup_{k \in  [i^*-1]} J_k$ be the subset of all elements in $\OPT$ 
of profits greater than $\eps^{i^*-1} \cdot \OPT(I)$, and $Q = \OPT \setminus (L \cup J_{i^*})$. 
To complete the proof of the lemma, we need several claims.
\begin{claim}
	\label{clam:Iq}
	$L \in \cm_{\leq q(\eps)}$. 
\end{claim}
%
\begin{claimproof}
	Since $L \subseteq \OPT$, by the hereditary property of $\cm$ we have that $L \in  \cm$. Also, 
	%
	\begin{equation*}
		\label{contradiction1}
		|L| \leq \sum_{e \in L} \frac{p(e)}{\eps^{i^*-1} \cdot \OPT(I)} = \frac{p(L)}{\eps^{i^*-1} \cdot \OPT(I)} \leq  \eps^{- (i^{*}-1)}  \leq   \eps^{-N+1} \leq \eps^{-\eps^{-1}} =  q(\eps)
	\end{equation*} The first inequality holds since $p(e) \geq  \eps^{i^*-1} \cdot \OPT$
	for all $e \in L$. For the second inequality, we note that $L$ is a solution for $I$. By the above it follows that $L \in \cm_{\leq q(\eps)}$. 
\end{claimproof} 
By Claim~\ref{clam:Iq} and as $R$ is a representative set,
it follows that $L$ has a replacement $Z_L \subseteq R$. 
Let $\Delta_L = (L \setminus H) \cup Z_L$. By Property~\ref{p:I} of Definition~\ref{def:Replacement}, we have that $\Delta_L \in \cm_{\leq q(\eps)}$, and it also holds that $\cm_{\leq q(\eps)} \subseteq  \cm$. 
Hence, $\Delta_L \in  \cm$. Furthermore, as $Q \subseteq \OPT$ and  $\OPT \in \cm$, by the 
hereditary property for $\cm$ we have that $Q \in  \cm$. Therefore, by Lemma~\ref{ob:matroid}, there is a subset $T \subseteq Q \setminus\Delta_L$, where $|T|  = \max\{|Q| - 2 \cdot |\Delta_L|,0\}$, such that $\Delta_L \cup T \in \cm$. 

Let $S = \Delta_L \cup T$. We show that $S$ satisfies the conditions of the lemma. 

\begin{claim}
	\label{claim:IsSolution}
	$S$ is a solution for $I$. 
\end{claim}

\begin{claimproof}
	By the definition of $T$ it holds that $S = \Delta_L \cup T \in \cm$. Moreover, 	
	\[
	\begin{array}{ll}
		w(S) &= w(\Delta_L\cup T) \\
		& \leq w(Z_L)+ w(L \setminus H) +w(T) \\
		& \leq w(L \cap H)+w(L \setminus H)+w(T) \\ 
		& \leq w(L)+w(Q) \\ 
		& \leq w(\OPT)\\
		& \leq \beta.
	\end{array}
	\]
	The second inequality holds since $w(Z_L) \leq w(L \cap H)$ (see Property~\ref{p:s} of Definition~\ref{def:Replacement}). For the third inequality, recall that $T \subseteq Q$. The last inequality holds since $\OPT$ is a solution for $I$. 
\end{claimproof} 

The proof of the next claim relies on
the {\em profit gap}  between the elements in $Q$ and $L$. 
\begin{claim}
	\label{clam:profitBound1}
	$p\left(Q \setminus T\right) \leq \eps \cdot \OPT(I)$.
\end{claim}
\begin{claimproof} 
	
	Observe that 
	\begin{equation}
		\label{eq:menS}
		|Q \setminus T| \leq 2 \cdot |\Delta_L| \leq 2 \cdot |Z_L|+2 \cdot |L \setminus H| \leq 2 \cdot |L \cap H|+2 \cdot |L \setminus H| \leq 2 \cdot |L|.
	\end{equation} 
	The first inequality follows from the definition of $T$. For the third inequality, we use Property~\ref{p:car} of Definition~\ref{def:Replacement}. Hence, 
	\begin{equation*}
		\begin{aligned}
			p(Q \setminus T) \leq{} & |Q \setminus T| \cdot \eps^{i^*} \cdot \OPT(I) \leq  2 \cdot |L| \cdot \eps^{i^*} \cdot \OPT(I) \leq 2\eps \cdot p(L) \leq 2\eps \cdot \OPT(I).
		\end{aligned}
	\end{equation*} 
	
	The first inequality holds since $p(e) \leq \eps^{i^*} \cdot \OPT(I)$ for all $e \in Q$. 
	%
	The second inequality is by \eqref{eq:menS}. The third inequality holds since $p(e) > \eps^{i^*-1} \cdot \OPT(I)$ for all $e \in L$. 
\end{claimproof} 	

\begin{claim}
	\label{clam:profitBound2}
	$p\left(S\right) \geq (1-4\eps) \OPT(I)$.
\end{claim} 

\begin{claimproof} 
	%
	By Property~\ref{p:p} of Definition~\ref{def:Replacement},
	\begin{equation}
		\label{eq:proofProfit1}
		\begin{aligned}
			p(\Delta_L) ={} & p((L \setminus H) \cup Z_L) \geq (1-\eps) \cdot p(L).
		\end{aligned}
	\end{equation} Moreover, 
	\begin{equation}
		\label{eq:proofProfit2}
		\begin{aligned}
			p(T) {} & \geq p(Q) - p(Q \setminus T) \geq p(Q) - 2\eps \cdot \OPT(I) \geq (1-\eps) \cdot p(Q) - 2\eps \cdot \OPT(I). 
		\end{aligned}
	\end{equation} 
	
	The second inequality is by Claim~\ref{clam:profitBound1}. Using \eqref{eq:proofProfit1} and \eqref{eq:proofProfit2}, we have that 
	
	\[	
	\begin{array}{ll}
		p(\Delta_L)+p(T) & \geq (1-\eps) \cdot p(L \cup Q)-2\eps \cdot \OPT(I) 
		\\ & = (1-\eps) \cdot p(\OPT \setminus J_{i^*})-2\eps \cdot \OPT(I) \\
		&  \geq (1-\eps) \cdot (1-\eps) \cdot \OPT(I)-2\eps \cdot \OPT(I)\\
		&  \geq (1-4\eps) \cdot \OPT(I). 
	\end{array}
	\]
	
	The second inequality holds since $p(J_{i^*}) \leq \eps \cdot \OPT(I)$. Observe that 
	$S = \Delta_L \cup T$ and $T \cap \Delta_L = \emptyset$. Therefore,  $$p(S) = p(\Delta_L)+p(T) \geq (1-4\eps) \cdot \OPT(I).$$
	
\end{claimproof} 
Finally, we note that, by \eqref{J_i} and the definition of $Q$, it holds that $Q \cap H = \emptyset$. Consequently, by the definition of $S$, we have that $S \cap H \subseteq Z_L$. 
As $Z_L \subseteq R$ (by Definition~\ref{def:Representatives}), it follows that $S \cap H \subseteq R$. Hence, using Claims~\ref{claim:IsSolution} and~\ref{clam:profitBound2},
we have the statement of the lemma.  \qed
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


{\bf Proof of Lemma~\ref{lem:sufficientRep}:}
	For the proof of the lemma, we define a {\em substitution} of some independent set as in \cite{doron2022eptas}. The first two properties of substitution of some $G \in \cm_{\leq q(\eps)}$ are identical to the first two properties in the definition of a replacement of $G$. 
	However, we require that a substitution preserves the number of profitable elements in $G$ from each profit class, and that a substitution must be disjoint to the set of non-profitable elements in $G$. %
	
	\begin{definition}
		\label{def:sub}
		For $G \in \cm_{\leq q(\eps)}$ and $Z_G \subseteq \bigcup_{r \in [\log_{1-\eps} \left(\frac{\eps}{2}\right)+1] } C_r(\alpha)$, we say that $Z_G$ is a {\em substitution} of $G$ if the following holds. \begin{enumerate}
			
			
			\item $(G \setminus H) \cup Z_G \in \cm_{\leq q(\eps)}$.\label{pp:1}
			
			\item  $w(Z_G) \leq w(G \cap H)$.\label{pp:2}
			
			\item For all $r \in [\log_{1-\eps} \left(\frac{\eps}{2}\right)+1]$ it holds that $|C_r(\alpha) \cap Z_G| = |C_r(\alpha) \cap G \cap H|$.\label{pp:3} 
			
			
			\item $(G \setminus H) \cap Z_G = \emptyset$.\label{pp:4}
			%
		\end{enumerate}
	\end{definition}
	\begin{claim}
		\label{claim:substitution}
		For any $G \in \cm_{\leq q(\eps)}$ there is a substitution $Z_G$ of $G$ such that $Z_G \subseteq R$. 
	\end{claim}
	\begin{claimproof}
		Let $G \in \cm_{\leq q(\eps)}$ and let $Z_G$ be a substitution of $G$ such that $|Z_G \cap R|$ is maximal among all substitutions of $G$; formally, let $\mathcal{S}(G)$ be all substitutions of $G$ and let $Z_G \in \{ Z \in \mathcal{S}(G)~|~ |Z \cap R| = \max_{Z' \in \mathcal{S}(G)} |Z' \cap R|\}$. Since $G \cap H$ is in particular a substitution of $G$  it follows that $\mathcal{S}(G)\neq \emptyset$, and thus  $Z_G$ is well defined.  Assume towards a contradiction that there is $a \in Z_G \setminus R$; then, by Definition~\ref{def:sub} there is $r \in [\log_{1-\eps} \left(\frac{\eps}{2}\right)+1]$ such that $a \in C_r(\alpha)$. Let $\Delta_G = (G \setminus H) \cup Z_G$; by definition~\ref{def:sub} it holds that $\Delta_G \in \cm_{\leq q(\eps)}$. In addition, because $R$ is exchangeable for $I,\eps,\alpha$, and $r$, by Definition~\ref{def:r-set} there is $b \in C_r(\alpha) \cap R \setminus \Delta_G$ such that $w(b) \leq w(a)$ and $\Delta_G -a+b \in \cm_{\leq q(\eps)}$. Then,  the properties of Definition~\ref{def:sub} are satisfied for $Z_G-a+b$ by the following. \begin{enumerate}
			\item $(G\setminus H) \cup (Z_G -a +b) =  \Delta_G-a+b \in \cm_{\leq q(\eps)}$ by the definition of $b$. 
			
			\item  $w(Z_G-a+b) \leq w(Z_G) \leq w(G\cap H)$ because $w(b) \leq w(a)$. 
			
			\item for all $r' \in [\log_{1-\eps} \left(\frac{\eps}{2}\right)+1]$ it holds that $|C_{r'}(\alpha) \cap (Z_G-a+b)| = |C_{r'}(\alpha) \cap Z_G| = |C_{r'}(\alpha) \cap G \cap H|$ because $a,b \in C_r(\alpha)$.
			
			\item $|(G \setminus H) \cap (Z_G -a+b)| \leq |(G \setminus H) \cap (Z_G)| = 0$ where the inequality follows because $b \notin \Delta_G$ and the equality is since $Z_G$ is a substitution of $G$. 
		\end{enumerate}
		
		By the above and Definition~\ref{def:sub}, it follows that $Z_G+a-b$ is a substitution of $G$; that is, $Z_G+a-b \in \mathcal{S}(G)$. Moreover, \begin{equation}
			\label{eq:ZG}
			|R \cap (Z_G -a+b)|>|R \cap Z_G| = \max_{Z \in \mathcal{S}(G)} |Z \cap R|.
		\end{equation} The first inequality is because $a \in Z_G \setminus R$ and $b \in R$. By \eqref{eq:ZG} we reach a contradiction since we found a substitution of $G$ with more elements in $R$ than $Z_G \in \mathcal{S}(G)$, which is defined as a substitution of $G$ with maximal number of elements in $R$. Therefore, $Z_G \subseteq R$ as required.
		\end{claimproof}
	 %$Z_G \in \mathcal{S}(G)$. 
	%


\begin{claim}
	\label{claim:RR}
	For all $e \in H$ there is exactly one $r \in [\log_{1-\eps} \left(\frac{\eps}{2}\right)+1]$ such that $e \in C_r(\alpha)$.
\end{claim}
\begin{claimproof}
	Let $e \in H$. Observe that: \begin{equation}
		\label{eq:app}
		\frac{\eps}{2} \leq \frac{p(e)}{2 \cdot \OPT(I)} \leq \frac{p(e)}{2 \cdot \alpha} \leq \frac{p(e)}{\OPT(I)} \leq 1.
	\end{equation}The first inequality holds since $e \in H$. The second and third inequalities are because $\alpha$ is the value of a $2$-approximation for the optimum of $I$; thus, $\frac{\OPT(I)}{2} \leq \alpha \leq \OPT(I)$. The last inequality is because $\{e\}$ is a solution of $I$ (or this element can be discarded from the instance as it cannot appear in any solution of $I$). In addition, observe that for $r_0 = \ceil{\log_{1-\eps} \frac{\eps}{2}}$ it holds that $(1-\eps)^{r_0} \leq \frac{\eps}{2}$ and that for $r_1 = 1$ it holds that $(1-\eps)^{r_1-1} = 1$. Hence, because $r_0 \leq \floor{\log_{1-\eps} \left(\frac{\eps}{2}\right)+1}$, by \eqref{eq:app}, there is exactly one $r \in [\log_{1-\eps} \left(\frac{\eps}{2}\right)+1]$ such that $\frac{p(e)}{2\alpha} \in \big((1-\eps)^r, (1-\eps)^{r-1}\big]$; thus, by \eqref{Er} it holds that $e \in C_r(\alpha)$ and $e \notin C_{r'}(\alpha)$ for $r' \in [\log_{1-\eps} \left(\frac{\eps}{2}\right)+1] \setminus \{r\}$.  
\end{claimproof}

We are now ready to prove Lemma~\ref{lem:sufficientRep}. The proof follows by showing that for any $G \in \cm_{\leq q(\eps)}$ a substitution of $G$ which is a subset of $R$ is in fact a replacement of $G$. Let $G \in \cm_{\leq q(\eps)}$; by Claim~\ref{claim:substitution}, $G$ has a substitution $Z_G \subseteq R$. Then, \begin{equation}
	\label{eq:profitR}
	\begin{aligned}
		p(Z_G) \geq{} & \sum_{r \in [\log_{1-\eps} \left(\frac{\eps}{2}\right)+1]} p(C_r(\alpha) \cap Z_G) 
		\\ \geq{} &  \sum_{r \in [\log_{1-\eps} \left(\frac{\eps}{2}\right)+1] \text{ s.t. } C_r(\alpha) \neq \emptyset} |C_r(\alpha) \cap Z_G| \cdot \min_{e \in C_r(\alpha)} p(e) 
		\\ \geq{} & \sum_{r \in [\log_{1-\eps} \left(\frac{\eps}{2}\right)+1] \text{ s.t. } C_r(\alpha) \neq \emptyset} |C_r(\alpha) \cap G \cap H| \cdot (1-\eps) \cdot \max_{e \in C_r(\alpha)} p(e) 
		\\ \geq{} & (1-\eps) \cdot p(G \cap H).
	\end{aligned}
\end{equation}  The third inequality is by \eqref{Er} and Property~\ref{pp:3} of Definition~\ref{def:sub}. The last inequality follows from Claim~\ref{claim:RR}. Therefore,  
\begin{equation}
	\label{eq:profitFINAL}
	\begin{aligned}
		p((G \setminus H) \cup Z_G) & = p(G \setminus H)+p(Z_G) \\
		&  \geq p(G \setminus H)+(1-\eps) \cdot p(G \cap H) \\
		& \geq (1-\eps) \cdot p(G).
	\end{aligned}
\end{equation}
The first equality follows by Property~\ref{pp:4} of Definition~\ref{def:sub}. The first inequality is by \eqref{eq:profitR}. Now,  $Z_G$ satisfies Property~\ref{p:I} and~\ref{p:s} of Definition~\ref{def:Replacement} by Properties~\ref{pp:1},~\ref{pp:2} of Definition~\ref{def:sub}, respectively. In addition, $Z_G$ satisfies Property~\ref{p:p} of Definition~\ref{def:Replacement} by \eqref{eq:profitFINAL}. Finally, $Z_G$ satisfies Property~\ref{p:car}  of Definition~\ref{def:Replacement} by $$|Z_G| = \sum_{r \in [\log_{1-\eps} \left(\frac{\eps}{2}\right)+1]} |Z_G \cap C_r(\alpha)| \leq \sum_{r \in [\log_{1-\eps} \left(\frac{\eps}{2}\right)+1]} |G \cap H \cap C_r(\alpha)| = |G \cap H|.$$ The first inequality holds since $Z_G$ is a substitution of $G$. The last equality follows from Claim~\ref{claim:RR}. We conclude that $Z_G$ is a replacement of $G$ such that $Z_G \subseteq R$; thus, $R$ is a representative set by Definition~\ref{def:Representatives}. \qed











	In the following proofs we rely on the next technical auxiliary claim. \begin{claim}
	\label{claim:log}
	For all $0<\eps<\frac{1}{2}$ it holds that $\log_{1-\eps} \left(\frac{\eps}{2}\right)+1 \leq 3 \eps^{-2}$.
\end{claim}
\begin{claimproof}
	Using logarithm rules we have
	% 
	\begin{equation*}
		\label{eq:log1}
		\log_{1-\eps} \left(\frac{\eps}{2}\right)+1  \leq 
		%
		\frac{\ln \left(\frac{2}{\eps}\right)}{-\ln \left(1-\eps \right)}+1 \leq \frac{2\eps^{-1}}{\eps}+1 \leq 3 \eps^{-2}. 
	\end{equation*} 
	The second inequality follows from  $x< -\ln (1-x), \forall x>-1, x \neq 0$, and $\ln (y) < y, \forall y>0$. 
\end{claimproof}





{\bf Proof of Lemma~\ref{lem:main}:}
	Let $\alpha$ be the result of Step~\ref{step:REPalpha} of Algorithm~\ref{alg:findRep} and let $r \in  [\log_{1-\eps} \left(\frac{\eps}{2}\right)+1]$. We split the proof into two complementary cases depending on the type of constraint of $I$. \begin{itemize}
		\item $\cC$ is a matching constraint. Then, by Lemma~\ref{lem:mainMatching} it holds that $ \textsf{RepMatching}(\cI,\eps,\alpha,r)$ is an exchangeable set for $I,\eps,\alpha$, and $r$ such that $\left|     \textsf{RepMatching}(\cI,\eps,\alpha,r)    \right| \leq 80 \cdot {q(\eps)}^3$. Therefore, by Step~\ref{step:REPforr}, Step~\ref{step:match}, and Step~\ref{step:REPret} of Algorithm~\ref{alg:findRep} it holds that $R$ is an exchangeable set for $I,\eps,\alpha$, and for all $r \in  [\log_{1-\eps} \left(\frac{\eps}{2}\right)+1]$ such that $|R| \leq \left( \log_{1-\eps} \left(\frac{\eps}{2}\right)+1\right)  \cdot 80 \cdot q(\eps)^3$.  Then, by Definition~\ref{def:r-set} and Lemma~\ref{lem:sufficientRep} it holds that $R$ is a representative set of $I$ and $\eps$. Moreover, the running time of the algorithm is $\textnormal{poly}(|I|)$ in this case. Step~\ref{step:REPAPP} can be computed in time $\textnormal{poly}(|I|)$ using a PTAS for BC with
		an error parameter $\eps= \frac{1}{2}$ (see~\cite{BBGS11}). In addition, each iteration of the \textbf{for} loop of Step~\ref{step:REPforr} can be computed in time $\textnormal{poly}(|I|)$ by Lemma~\ref{lem:mainMatching}. Hence, as we have $O\left(\log_{1-\eps} \left(\frac{\eps}{2}\right)\right) $ iterations of the  \textbf{for} loop of Step~\ref{step:REPforr} , the running time of the algorithm is $O\left(\log_{1-\eps} \left(\frac{\eps}{2}\right)\right)  \cdot \textnormal{poly}(|I|)$; then, by Claim~\ref{claim:log} the running time is $O(\eps^{-2}) \cdot  \textnormal{poly}(|I|)$  in case that $\cC$ is a matching constraint.
		
		\item $\cC$ is a matroid intersection constraint. By Lemma~\ref{lem:mainMatroid}, $\textsf{RepMatroidIntersection}(\cI,\eps,\alpha,r)$ is an exchangeable set for $I,\eps,\alpha$, and $r$ such that $\left|     \textsf{RepMatroidIntersection}(\cI,\eps,\alpha,r)    \right| \leq {q(\eps)}^{O(q(\eps))}$. Therefore, by Step~\ref{step:REPforr}, Step~\ref{step:matroid}, and Step~\ref{step:REPret} of Algorithm~\ref{alg:findRep} it holds that $R$ is an exchangeable set for $I,\eps,\alpha$, for all $r \in  [\log_{1-\eps} \left(\frac{\eps}{2}\right)+1]$ such that $|R| \leq \left( \log_{1-\eps} \left(\frac{\eps}{2}\right)+1\right)  \cdot  {q(\eps)}^{O(q(\eps))}$.  Then, by Definition~\ref{def:r-set} and Lemma~\ref{lem:sufficientRep} it holds that $R$ is a representative set of $I$ and $\eps$. For the running time of the algorithm, observe that Step~\ref{step:REPAPP} can be computed in time $\textnormal{poly}(|I|)$ using a PTAS for BC with
		an error parameter $\eps= \frac{1}{2}$ (see~\cite{BBGS11}). In addition, each iteration of the \textbf{for} loop of Step~\ref{step:REPforr} can be computed in time ${q(\eps)}^{O(q(\eps))} \cdot \textnormal{poly}(|I|)$ by Lemma~\ref{lem:mainMatroid}. Hence, as we have $O\left(\log_{1-\eps} \left(\frac{\eps}{2}\right)\right) $ iterations of the  \textbf{for} loop of Step~\ref{step:REPforr} , the running time of the algorithm is $O\left(\log_{1-\eps} \left(\frac{\eps}{2}\right)\right)  \cdot {q(\eps)}^{O(q(\eps))} \cdot \textnormal{poly}(|I|)$; then, by Claim~\ref{claim:log} it holds that $O\left(\log_{1-\eps} \left(\frac{\eps}{2}\right)\right) = O(\eps^{-2})$ and it follows that $O\left(\log_{1-\eps} \left(\frac{\eps}{2}\right)\right)  = {q(\eps)}^{O(1)}$; thus, the running time of the algorithm is $ {q(\eps)}^{O(q(\eps))} \cdot \textnormal{poly}(|I|)$ and it also follows that $|R| \leq {q(\eps)}^{O(q(\eps))}$ in case that $\cC$ is a matroid intersection constraint. \qed
	\end{itemize}
	










For the proof of Lemma~\ref{thm:EPTAS}, we use the following auxiliary lemmas.  

\begin{lemma}
	\label{thm:aux1}
	Given a \textnormal{BC} instance $I = (E, \cC, w,p, \beta)$ and $0<\eps<\frac{1}{2}$, Algorithm~\ref{alg:EPTAS} returns a solution for $I$ of profit at least $(1-8\eps) \cdot \OPT(I)$.
\end{lemma}

\begin{proof}

	By Lemma~\ref{lem:Solution},  there is a solution $S$ for $I$ such that $S \cap H \subseteq R$, and $p\left(S\right) \geq (1-4\eps) \OPT(I)$. As for all $e \in S \cap H$ we have $p(e) > \eps \cdot \OPT(I)$, and $S$ is a solution for $I$, it follows that $|S \cap H| \leq \eps^{-1}$.
	% Then, by Step~\ref{step:for} of Algorithm~\ref{alg:EPTAS} 
	We note that there is an iteration of Step~\ref{step:for} in which $F = S \cap H$; thus, in Step~\ref{step:vertex} we construct a solution ${\lambda}^{S \cap H}$ of $I_{S \cap H}$ such that: %We use $X(A) = \{e \in E(\alpha) \setminus A~|~ \bar{\lambda}^{A}_e = 1\}$ for every basic solution $\bar{\lambda}^{A}$ computed in Step~\ref{step:vertex} for $A \subseteq R$.  
	\begin{equation}
		\label{eq:finalProfitA}
		\begin{aligned}
			p\left(\lambda^F\right) \geq \OPT(I_{S \cap H})-2 \cdot \max_{e \in E_{S \cap H}} p(e) \geq p(S \setminus H)- 2 \cdot \max_{e \in E_{S \cap H}} p(e) \geq p(S \setminus H)-4\eps \cdot \OPT(I). 
		\end{aligned}
	\end{equation}
	%The first inequality holds since $S \setminus H$ is in particular a solution of the extension instance $I_F$ by Definition~\ref{def:instance}. 
	The first inequality holds by Lemma~\ref{lem:grandoni}. The second inequality holds since $S \setminus H$ is in particular a solution of the extension instance $I_F$ by Definition~\ref{def:instance}. The third inequality holds since for all $e \in E(S \cap H)$ it holds that $p(e) \leq 2\eps \cdot \alpha \leq 2 \eps \cdot \OPT(I)$. Now, recall $K_{S \cap H}$ defined in Step~\ref{step:Cf} of Algorithm~\ref{alg:EPTAS}. 
	\begin{equation}
		\label{eq:finalProfit}
		\begin{aligned}
			p(K_{S \cap H}) ={} & p(S \cap H)+p\left(\lambda^F\right)  \geq  p(S)- 4\eps \cdot \OPT(I) \geq (1-8\eps) \OPT(I).
		\end{aligned}
	\end{equation}
	
	The first inequality uses~\eqref{eq:finalProfitA}. The last inequality is by Lemma~\ref{lem:Solution}.   \begin{claim}
		\label{claim:Cf}
		$A  = \textnormal{\textsf{EPTAS}}(\cI,\eps)$ is a solution of $I$. 
	\end{claim}
	%
	\begin{claimproof} If $A = \emptyset$ the claim trivially follows since $\emptyset$ is a solution of $I$. Otherwise, by Step~\ref{step:update} of Algorithm~\ref{alg:EPTAS}, there is a solution $F$ of $I$ such that $A = K_F$. Observe that by Definition~\ref{def:instance} it holds that $\lambda^F \in \cm(\cC_F)$ and that $\lambda^F \cup F \in \cm(\CC)$; thus, it holds that $K_F \in \cm(\cC)$. Additionally, 
		
		
		%By Observation~\ref{ob:convexHull}, $X(F)$ is an independent set in the matroid $M_{F}(\alpha)$. 
		%Also, recall that $\cm_{F} (\alpha) = \left((E,\cI) /F \right) \cap E(\alpha) $. Hence, by Definition~\ref{def:matroids}, we have that $X(F) \cup F =K_F \in \cI$. 
		
		
		
		%
		$$w\left(K_{F}\right) = w(F)+w\left(\lambda^F\right) = w(F)+ w_F(\lambda^F) \leq w(F)+\beta_F = w(F)+\beta-w(F) = \beta.$$ 
		The inequality is since $\lambda^F$ is a solution for $I_F$. By the above, we conclude that $A$ is a solution for $I$.  
	\end{claimproof} 
	
	By Claim~\ref{claim:Cf}, Steps~\ref{step:for}, \ref{step:update} and~\ref{step:retA}
	of Algorithm~\ref{alg:EPTAS} and \eqref{eq:finalProfit}, we have that
	%
	$A = \textsf{EPTAS}(I,\eps)$ is a solution for $I$ satisfying $p(A) \geq p(K_{S \cap H}) \geq (1-8\eps) \OPT(I)$. This completes the proof. 	
\end{proof}
























%{\bf Proof of Lemma~\ref{thm:running}:}

\begin{lemma}
	\label{thm:aux2}
	Given a \textnormal{BC} instance $I = (E, \cC, w,p, \beta)$ and $0<\eps<\frac{1}{2}$, the running time of Algorithm~\ref{alg:EPTAS} satisfies one of the following. \begin{itemize}
		\item If $\cC$ is a matroid intersection constraint the running time is ${q(\eps)}^{O(\eps^{-1} \cdot q(\eps))} \cdot \textnormal{poly}(|I|)$. 
		
		\item  If $\cC$ is a matching constraint  the running time is $2^{ O \left(\eps^{-2} \log \frac{1}{\eps} \right)} \cdot \textnormal{poly}(|I|)$.
	\end{itemize}
\end{lemma}
\begin{proof}


	For the following, let $$W = 	\big\{F \subseteq R~\big|~ |F| \leq \eps^{-1}, F \in \cm(\cC), w(F) \leq \beta\big\}$$ be the set of solutions considered in Step~\ref{step:for} of Algorithm~\ref{alg:EPTAS}. We split the proof into two parts, based on the type of constraints of $I$. \begin{enumerate}
		\item $\cC$ is a matroid intersection constraint. By Lemma~\ref{lem:main}, the time complexity of Step~\ref{step:rep} 
		%
		is ${q(\eps)}^{O(q(\eps))}  \cdot \textnormal{poly}(|I|)$. In addition, Step~\ref{step:APP2} can be computed in time $\textnormal{poly}(|I|)$, by using a PTAS for BC taking 
		%with parameter 
		$\eps=\frac{1}{2}$ (see~\cite{GZ10}). 
	% Now, Let $$W = 	\big\{F \subseteq R~\big|~ |F| \leq \eps^{-1}, F \in \cm(\cC), c(F) \leq \beta\big\}$$ be the set of solutions considered in Step~\ref{step:for} of Algorithm~\ref{alg:EPTAS}. 
	Then,
		\begin{equation}
			\label{eq:subR11111}
			\begin{aligned}
				|W| \leq{} &  \left(|R|+1\right)^{\eps^{-1}}
				\leq  {\left({q(\eps)}^{O(q(\eps))}\right)}^{\eps^{-1}} = {q(\eps)}^{O(\eps^{-1} \cdot q(\eps))}.
			\end{aligned}
		\end{equation} The second inequality is by Lemma~\ref{lem:main}. Hence, by \eqref{eq:subR11111}, the number of iterations of the {\bf for} loop  in Step~\ref{step:for} is bounded by ${q(\eps)}^{O(\eps^{-1} \cdot q(\eps))}$. In addition, by Lemma~\ref{lem:grandoni}, the running time of each iteration is  $\textnormal{poly}(|I|)$. By the above, the running time of Algorithm~\ref{alg:EPTAS} is ${q(\eps)}^{O(\eps^{-1} \cdot q(\eps))} \cdot \textnormal{poly}(|I|)$  If $\cC$ is a matroid intersection constraint.  
		
		
		
		\item 	$\cC$ is a matching constraint. By Lemma~\ref{lem:main}, the time complexity of Step~\ref{step:rep} 
		%
		is $\textnormal{poly}(|I|)$. Step~\ref{step:APP2} can be computed in time $\textnormal{poly}(|I|)$, by using a PTAS for BC taking 
		%with parameter 
		$\eps=\frac{1}{2}$ (see~\cite{GZ10}). Therefore, \begin{equation}
			\label{eq:R}
			|R| \leq \left(\log_{1-\eps} \left(\frac{\eps}{2}\right)+1\right)  \cdot 80 \cdot q(\eps)^3 \leq 3\eps^{-2} \cdot 80 \eps^{-3\eps^{-1}} \leq 240 \cdot \eps^{-4\eps^{-1}}. 
		\end{equation}
		The first inequality is by Lemma~\ref{lem:main} and that the number of  iterations of the {\bf for} loop  in Step~\ref{step:for} is bounded by $ \left(\log_{1-\eps} \left(\frac{\eps}{2}\right)+1\right)$. The second inequality is by Claim~\ref{claim:log}. Then,
		\begin{equation}
			\label{eq:subR}
			\begin{aligned}
				|W| \leq{} &  \left(|R|+1\right)^{\eps^{-1}}
				\leq  {\left(240 \cdot \eps^{-4\eps^{-1}}+1\right)}^{\eps^{-1}}
				\leq {\left(\eps^{-20\eps^{-2}}\right)} = 2^{ O \left(\eps^{-2} \log \frac{1}{\eps} \right)}.
			\end{aligned}
		\end{equation} The second inequality is by \eqref{eq:R}. Hence, by \eqref{eq:subR}, the number of iterations of the {\bf for} loop  in Step~\ref{step:for} is bounded by $2^{ O \left(\eps^{-2} \log \frac{1}{\eps} \right)}$. In addition, by Lemma~\ref{lem:grandoni}, the running time of each iteration is  $\textnormal{poly}(|I|)$. By the above, the running time of Algorithm~\ref{alg:EPTAS} is $2^{ O \left(\eps^{-2} \log \frac{1}{\eps} \right)} \cdot \textnormal{poly}(|I|)$  If $\cC$ is a matching constraint.  
	\end{enumerate} \end{proof}


{\bf Proof of Lemma~\ref{thm:EPTAS}:} The proof follows by Lemma~\ref{thm:aux1} and Lemma~\ref{thm:aux2}. \qed







==> findRep.tex <==
\section{Properties of \textsf{FindRep}}
\label{sec:findRep}
